Continual Learners are Incremental Model Generalizers

Motivated by the efficiency and rapid convergence of pre-trained models for solving downstream tasks, this paper extensively studies the impact of Continual Learning (CL) models as pre-trainers. In both supervised and unsupervised CL, we find that the transfer quality of the representation often increases gradually without noticeable degradation in fine-tuning performance. This is because CL models can learn improved task-general features when easily forgetting task-specific knowledge. Based on this observation, we suggest a new unsupervised CL framework with masked modeling, which aims to capture fluent task-generic representation during training. Furthermore, we propose a new fine-tuning scheme, GLobal Attention Discretization (GLAD), that preserves rich task-generic representation during solving downstream tasks. The model fine-tuned with GLAD achieves competitive performance and can also be used as a good pre-trained model itself. We believe this paper breaks the barriers between pre-training and fine-tuning steps and leads to a sustainable learning framework in which the continual learner incrementally improves model generalization, yielding better transfer to unseen tasks.

==> materials/figures/5_ft_visualization.tex <==
% \begin{figure*}%[h!]
%     \centering
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{cc}
%     \includegraphics[height=3.cm]{figures/20220902_scl_si_per_task.PNG}&\hspace{-0.1in}
%     \includegraphics[height=3.cm]{a.pdf}\\
%     \end{tabular}}
%     \vspace{-0.1in}
%     \caption{\footnotesize \bf Performance decreases during CL (straightforward) - Left.}
%     \label{fig:main_fig}
%     \vspace{-0.25in}
% \end{figure*}
\begin{wrapfigure}{rt!}{0.5\textwidth}
\vspace{-0.1in} % -0.35in
%     \hspace{-0.1in}
    \centering
    \begin{minipage}[t]{1.\textwidth}
        \includegraphics[height=2.8cm]{figures/20220902_scl_si_per_task.PNG}&
        \includegraphics[height=2.8cm]{figures/20220902_scl_si_per_task.PNG}\\
    \vspace{-0.3in}
    \end{minipage}\label{fig:supervised-pertask}
    \caption{\footnotesize \textbf{Performance decreases during SCL} straightforward.}
    \vspace{-0.1in}
\end{wrapfigure}

==> materials/figures/5_ours_attn_change.tex <==
\begin{figure*}%[h!]
    \footnotesize
    \centering
    \resizebox{.95\textwidth}{!}{%
    % \hspace{-0.2in}
    \begin{tabular}{ccc}    
    \includegraphics[align=c, height=3cm]{figures/attn_div/sup60_attn_diversity_attt0.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=3cm]{figures/attn_div/siam_attn_diversity_attt0.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=3cm]{figures/attn_div/mim_attn_diversity_attt0.png}
    \vspace{-0.1in}\\    
    \includegraphics[align=c, height=3cm]{figures/attn_div/sup60_entropy_diversity_attt0.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=3cm]{figures/attn_div/siam_entropy_diversity_attt0.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=3cm]{figures/attn_div/mim_entropy_diversity_attt0.png}
    \\
    \small{Supervised} &\hspace{-0.2in}
    \small{SimSiam} &\hspace{-0.2in}
    \small{SimMIM} \\
    \end{tabular}}
    \vspace{-0.1in}
    \caption{\footnotesize \bf The change of attention distance for first task (T0) and last task (T8) during continual representation learning.}
    \label{fig:ours-swin-attn}
    \vspace{-0.25in}
\end{figure*}

==> materials/figures/5_partial_freeze.tex <==
\begin{figure*}%[h!]
    \footnotesize
    \centering
    \resizebox{.95\textwidth}{!}{%
    % \hspace{-0.2in}
    \begin{tabular}{ccc}    
    \includegraphics[align=c, height=3cm]{figures/attn_div/sup60_attn_diversity_attt0.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=3cm]{figures/attn_div/siam_attn_diversity_attt0.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=3cm]{figures/attn_div/mim_attn_diversity_attt0.png}
    \small{Supervised} &\hspace{-0.2in}
    \small{SimSiam} &\hspace{-0.2in}
    \small{SimMIM} \\
    \end{tabular}}
    \vspace{-0.1in}
    \caption{\footnotesize \bf The change of attention distance for first task (T0) and last task (T8) during continual representation learning.}
    \label{fig:ours-swin-attn}
    \vspace{-0.25in}
\end{figure*}

==> materials/figures/5_swin_attn_single.tex <==
\begin{figure*}[t!]
    \small
    \centering
    \resizebox{1.05\textwidth}{!}{%    
    \hspace{-0.2in}
    \begin{tabular}{l@{\hspace{6pt}}cccccc}
    \rotatebox[origin=c]{90}{Supervised}\hspace{-0.1in}    
    &
    \includegraphics[align=c, height=1.9cm]{figures/sup/swin_attn_ep60/prtt0attt0.png}&\hspace{-0.25in}
    \includegraphics[align=c, height=1.9cm]{figures/sup/swin_attn_ep60/prtt8attt0.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=1.9cm]{figures/sup/swin_attn_ep60/prtt0attt9.png}&\hspace{-0.25in}
    \includegraphics[align=c, height=1.9cm]{figures/sup/swin_attn_ep60/prtt8attt9.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=1.9cm]{figures/sup/swin_entropy_ep60/prtt0attt9.png}&\hspace{-0.25in}
    \includegraphics[align=c, height=1.9cm]{figures/sup/swin_entropy_ep60/prtt8attt9.png}\\
    \rotatebox[origin=c]{90}{SimSiam}\hspace{-0.1in}    
    &
    \includegraphics[align=c, height=1.9cm]{figures/siam/swin_attn/prtt0attt0.png}&\hspace{-0.25in}
    \includegraphics[align=c, height=1.9cm]{figures/siam/swin_attn/prtt8attt0.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=1.9cm]{figures/siam/swin_attn/prtt0attt9.png}&\hspace{-0.25in}
    \includegraphics[align=c, height=1.9cm]{figures/siam/swin_attn/prtt8attt9.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=1.9cm]{figures/siam/swin_entropy/prtt0attt9.png}&\hspace{-0.25in}
    \includegraphics[align=c, height=1.9cm]{figures/siam/swin_entropy/prtt8attt9.png}\\
    \rotatebox[origin=c]{90}{SimMIM}\hspace{-0.1in}    
    & 
    \includegraphics[align=c, height=1.9cm]{figures/mim/swin_attn/prtt0attt0.png}&\hspace{-0.25in}
    \includegraphics[align=c, height=1.9cm]{figures/mim/swin_attn/prtt8attt0.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=1.9cm]{figures/mim/swin_attn/prtt0attt9.png}&\hspace{-0.25in}
    \includegraphics[align=c, height=1.9cm]{figures/mim/swin_attn/prtt8attt9.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=1.9cm]{figures/mim/swin_entropy/prtt0attt9.png}&\hspace{-0.25in}
    \includegraphics[align=c, height=1.9cm]{figures/mim/swin_entropy/prtt8attt9.png}
    \vspace{-0.05in}\\
    &
    \footnotesize $\bm{w}_{\bf{T0}}$ & \hspace{-0.25in}
    \footnotesize $\bm{w}_{\bf{T0 \rightarrow T8}}$ &\hspace{-0.2in}
    \footnotesize $\bm{w}_{\bf{T0}}$ &\hspace{-0.25in}
    \footnotesize $\bm{w}_{\bf{T0 \rightarrow T8}}$ &\hspace{-0.2in}
    \footnotesize $\bm{w}_{\bf{T0}}$ &\hspace{-0.25in}
    \footnotesize $\bm{w}_{\bf{T0 \rightarrow T8}}$
    \end{tabular}}
    \resizebox{0.95\textwidth}{!}{% 
    \hspace{0.15in} 
    \begin{tabular}{cccccc}      
    \multicolumn{2}{c}{\small (a) Attention Distance of \bf{T0}} & \hspace{0.2in}
    \multicolumn{2}{c}{\small (b) Attention Distance of \bf{T9}} & \hspace{0.2in}
    \multicolumn{2}{c}{\small (c) Attention Entropy of \bf{T9}}
    \end{tabular}}
    \vspace{-0.1in}
    \caption{\footnotesize \textbf{(a-b): Visualization of the attention distance} of an in-distribution (T0) and out-of-distribution task (T9) with respect to three continual pre-trained frameworks right after the completion of the first ($\bm{w}_{\bf{T0}}$) and last task ($\bm{w}_{\bf{T0\rightarrow T8}}$). \textbf{(c): Visualization of the entropy of each attention head's distribution} of unseen task T9.}
    \label{fig:swin-attn-entr-single}
    \vspace{-0.1in}
\end{figure*}

==> materials/figures/5_swin_entropy.tex <==
\begin{figure*}%[h!]
    \centering
    \resizebox{0.95\textwidth}{!}{%
    \hspace{-0.2in}
    \begin{tabular}{l@{\hspace{6pt}}cccccc}
    \rotatebox[origin=c]{90}{\footnotesize Supervised (ep60)}\hspace{-0.1in}    
    &
    \includegraphics[align=c, height=2.8cm]{figures/sup/swin_entropy_ep60/prtt0attt0.png}&\hspace{-0.3in}
    \includegraphics[align=c, height=2.8cm]{figures/sup/swin_entropy_ep60/prtt8attt0.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=2.8cm]{figures/sup/swin_entropy_ep60/prtt0attt8.png}&\hspace{-0.3in}
    \includegraphics[align=c, height=2.8cm]{figures/sup/swin_entropy_ep60/prtt8attt8.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=2.8cm]{aa.png}&\hspace{-0.3in}
    \includegraphics[align=c, height=2.8cm]{aa.png}\\
    % \rotatebox[origin=c]{90}{\footnotesize Supervised (ep100)}\hspace{-0.1in}    
    % &
    % \includegraphics[align=c, height=2.8cm]{figures/sup/swin_entropy_ep100/prtt0attt0.png}&\hspace{-0.3in}
    % \includegraphics[align=c, height=2.8cm]{figures/sup/swin_entropy_ep100/prtt8attt0.png}&\hspace{-0.2in}
    % \includegraphics[align=c, height=2.8cm]{figures/sup/swin_entropy_ep100/prtt0attt8.png}&\hspace{-0.3in}
    % \includegraphics[align=c, height=2.8cm]{figures/sup/swin_entropy_ep100/prtt8attt8.png}\\
    \rotatebox[origin=c]{90}{\footnotesize SimSiam}\hspace{-0.1in}    
    &
    \includegraphics[align=c, height=2.8cm]{figures/siam/swin_entropy/prtt0attt0.png}&\hspace{-0.3in}
    \includegraphics[align=c, height=2.8cm]{figures/siam/swin_entropy/prtt8attt0.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=2.8cm]{figures/siam/swin_entropy/prtt0attt8.png}&\hspace{-0.3in}
    \includegraphics[align=c, height=2.8cm]{figures/siam/swin_entropy/prtt8attt8.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=2.8cm]{aa.png}&\hspace{-0.3in}
    \includegraphics[align=c, height=2.8cm]{aa.png}\\
    \rotatebox[origin=c]{90}{\footnotesize SimMIM}\hspace{-0.1in}
    &
    \includegraphics[align=c, height=2.8cm]{figures/mim/swin_entropy/prtt0attt0.png}&\hspace{-0.3in}
    \includegraphics[align=c, height=2.8cm]{figures/mim/swin_entropy/prtt8attt0.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=2.8cm]{figures/mim/swin_entropy/prtt0attt8.png}&\hspace{-0.3in}
    \includegraphics[align=c, height=2.8cm]{figures/mim/swin_entropy/prtt8attt8.png}&\hspace{-0.2in}
    \includegraphics[align=c, height=2.8cm]{aa.png}&\hspace{-0.3in}
    \includegraphics[align=c, height=2.8cm]{aa.png}\\
    % \multicolumn{2}{c}{\footnotesize  (a) Supervised Learning} & \multicolumn{2}{c}{\footnotesize  (b) SimSiam (Contrastive)} & \multicolumn{2}{c}{\footnotesize  (b) SimMIM (Reconstruction)}\\
    &\multicolumn{2}{c}{\footnotesize  (a) Task 0} & \multicolumn{2}{c}{\footnotesize  (b) Task 8} & \multicolumn{2}{c}{\footnotesize  (b) Task 9} \\
    \end{tabular}}
    \vspace{-0.1in}
    \caption{\footnotesize \bf The change of attention entropy for first task (T0) and last task (T8) during continual representation learning.}
    \label{fig:swin-entr}
    \vspace{-0.25in}
\end{figure*}

==> materials/figures/5_transfer.tex <==
\begin{figure*}%[h!]
    \centering
    \footnotesize
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{cccc}
    \includegraphics[height=3.cm]{figures/transfer_sup_5eps.PNG}&\hspace{-0.1in}
    \includegraphics[height=3.cm]{figures/transfer_siam_5eps.PNG}&\hspace{-0.1in}
    \includegraphics[height=3.cm]{mim-678.pdf}&\hspace{-0.1in}
    \includegraphics[height=3.cm]{mim-ours678.pdf}\\
    % \multicolumn{2}{c}{\footnotesize  (a) Finetuning} & \multicolumn{2}{c}{\footnotesize  (b) Linear Probe} \\
    Supervised & Contrastive & Masked Model & Ours
    \end{tabular}}
    \vspace{-0.1in}
    \caption{\footnotesize \bf TBD}
    \label{fig:transfer}
    \vspace{-0.25in}
\end{figure*}

==> materials/table_vit_wd.tex <==
\begin{table*}[t]
\small
\centering
\caption{\small {\bf TBD} '\modify{*}' is running, '{*}' will run, '-' is N/A, the best and second-best performance are highlighted in '\bp{val}' and '\sbp{val}', respectively. We report the averaged performance across five independent runs in colored cells. Otherwise, the results are obtained from a single run. \label{tab:main_table1}}
%\setlength{\tabcolsep}{3pt} % 
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccc|cccc|cccc|cccc}
\toprule
{\textbf{\textsc{Vit-Tiny}}}&\multicolumn{4}{c}{\textsc{lr:0.02}} &\multicolumn{4}{c}{\textsc{lr:0.01}}&\multicolumn{4}{c}{\textsc{lr:0.005}} &\multicolumn{4}{c}{\textsc{lr:0.002}}\\
\midrule \textbf{\textsc{Finetune}}&
\textsc{Acc} &
\textsc{Fgt} &
\textsc{$a^T_{1,1}$} &
\textsc{$a^T_{N,N}$}&
\textsc{Acc} &
\textsc{Fgt} &
\textsc{$a^T_{1,1}$} &
\textsc{$a^T_{N,N}$}&
\textsc{Acc} &
\textsc{Fgt} &
\textsc{$a^T_{1,1}$} &
\textsc{$a^T_{N,N}$}&
\textsc{Acc} &
\textsc{Fgt} &
\textsc{$a^T_{1,1}$} &
\textsc{$a^T_{N,N}$}\\
\midrule
\textsc{w/o-rost-ep30-bs16}&&&&&&&&&&&&&\\
\textsc{lrd1e-2-wd0.1}&
*&*&*&*&
*&*&*&*&
39.72 & 44.05 & 80.20 & 90.53 &
*&*&*&*\\
\textsc{lrd1e-3-wd0.1}&
*&*&*&*&
*&*&*&*&
39.26 & 44.18 & 80.40 & 87.73 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.1}&
34.38 & 46.15 & 68.87 & 85.20 &
38.74 & 41.05 & 74.73 & 83.00 &
39.06 & 44.49 & 79.80 & 88.36 &
40.04 & 43.37 & 80.20 & 87.70 \\
&&&&&&&&&&&&&\\
\textsc{lrd1e-4-wd1.0}&
*&*&*&*&
*&*&*&*&
28.12 & 53.45 & 80.40 & 81.60 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.5}&
*&*&*&*&
*&*&*&*&
30.01 & 53.46 & 80.60 & 83.47 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.2}&
*&*&*&*&
*&*&*&*&
35.23 & 48.44 & 79.33 & 87.67 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.05}&
*&*&*&*&
*&*&*&*&
42.84 & 39.15 & 80.07 & 86.33 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.01}&
*&*&*&*&
*&*&*&*&
45.37 & 36.42 & 80.07 & 84.20 &
*&*&*&*\\
\midrule
\textsc{w/o-rost}&
\multicolumn{4}{c}{\textsc{ep50-bs16}}&
\multicolumn{4}{c}{\textsc{ep30-bs64}}&
\multicolumn{4}{c}{\textsc{ep50-bs64}}&
\multicolumn{4}{c}{\textsc{w/rost-ep50-bs64}}\\
\textsc{lrd1e-2-wd0.1}&
34.40 & 50.14 & 81.87 & 87.87 &
44.14 & 32.95 & 71.00 & 84.53 &
*&*&*&*&
*&*&*&*\\
\textsc{lrd1e-3-wd0.1}&
33.63 & 51.25 & 81.13 & 89.47 &
43.13 & 33.80 & 72.60 & 84.33 &
*&*&*&*&
*&*&*&*\\
\textsc{lrd1e-4-wd0.1}&
34.16 & 50.13 & 80.67 & 88.80 &
44.40 & 33.52 & 72.00 & 85.33 &
40.37 & 38.46 & 74.40 & 84.80 &
30.51 & 48.75 & 73.47 & 83.33 \\
&&&&&&&&&&&&&\\
\textsc{lrd1e-4-wd1.0}&
29.20 & 53.35 & 80.40 & 81.40 &
29.25 & 50.71 & 76.53 & 81.73 &
29.76 & 52.43 & 77.60 & 80.73 &
26.58 & 56.28 & 77.07 & 82.67 \\
\textsc{lrd1e-4-wd0.5}&
*&*&*&*&
*&*&*&*&
30.43 & 51.55 & 75.80 & 81.67 &
29.77 & 52.55 & 77.73 & 84.40 \\
\textsc{lrd1e-4-wd0.2}&
29.35 & 55.49 & 78.80 & 88.80 &
40.04 & 39.19 & 73.27 & 84.47 &
34.71 & 45.05 & 74.07 & 83.87 &
26.70 & 53.73 & 74.47 & 82.53 \\
\textsc{lrd1e-4-wd0.05}&
37.52 & 45.31 & 80.67 & 87.00 &
45.61 & 28.46 & 72.07 & 83.40 &
42.26 & 34.18 & 73.13 & 85.47 &
39.08 & 36.27 & 72.20 & 84.40 \\
\textsc{lrd1e-4-wd0.01}&
42.00 & 39.65 & 79.93 & 85.80 &
39.01 & 29.48 & 71.67 & 74.53 &
39.34 & 29.26 & 70.73 & 76.13 &
33.21 & 31.95 & 72.00 & 71.93 \\
\midrule
\textsc{w/-rost-ep30-bs16}&&&&&&&&&&&&&\\
\textsc{lrd1e-2-wd0.1}&
*&*&*&*&
33.29 & 46.34 & 73.93 & 83.33 &
32.01 & 51.53 & 79.07 & 87.73 &
*&*&*&*\\
\textsc{lrd1e-3-wd0.1}&
*&*&*&*&
32.08 & 47.67 & 74.40 & 82.73 &
29.78 & 54.07 & 80.20 & 87.73 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.1}&
28.96 & 51.36 & 69.53 & 83.60 &
29.40 & 50.96 & 75.60 & 84.20 &
30.90 & 52.78 & 80.00 & 87.33 &
33.18 & 50.25 & 78.93 & 86.13\\
&&&&&&&&&&&&&\\
\textsc{lrd1e-4-wd1.0}&
*&*&*&*&
26.41 & 55.38 & 80.13 & 81.13 &
24.43 & 57.45 & 80.90 & 81.50 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.5}&
*&*&*&*&
28.92 & 54.58 & 79.40 & 83.87 &
28.24 & 55.53 & 81.50 & 83.90 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.2}&
*&*&*&*&
29.86 & 51.22 & 76.67 & 83.67 &
31.26 & 52.52 & 80.90 & 87.00 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.05}&
*&*&*&*&
38.82 & 39.88 & 74.60 & 84.40 &
35.75 & 47.21 & 80.60 & 87.40 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.01}&
*&*&*&*&
40.57 & 31.40 & 73.60 & 77.93 &
40.46 & 41.01 & 80.00 & 84.93 &
*&*&*&*\\
\midrule
\textsc{w/-rost-ep50-bs16}&&&&&&&&&&&&&\\
\textsc{lrd1e-2-wd0.1}&
*&*&*&*&
29.19 & 51.42 & 76.00 & 82.80 &
30.11 & 53.47 & 80.00 & 87.73 &
*&*&*&*\\
\textsc{lrd1e-3-wd0.1}&
*&*&*&*&
31.00 & 48.64 & 77.07 & 82.00 &
27.80 & 56.51 & 78.73 & 88.00 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.1}&
*&*&*&*&
26.44 & 53.91 & 76.67 & 82.47 &
30.14 & 53.88 & 81.27 & 89.53 &
27.46 & 56.05 & 80.20 & 87.27\\
&&&&&&&&&&&&&\\
\textsc{lrd1e-4-wd1.0}&
*&*&*&*&
26.13 & 56.83 & 80.47 & 81.87 &
26.33 & 56.31 & 80.00 & 82.07 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.5}&
*&*&*&*&
23.80 & 61.45 & 80.60 & 84.93 &
30.30 & 53.94 & 81.40 & 85.87 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.2}&
*&*&*&*&
26.73 & 54.78 & 77.93 & 85.00 &
26.92 & 57.19 & 80.13 & 85.80 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.05}&
*&*&*&*&
32.34 & 47.72 & 75.80 & 83.47 &
33.33 & 49.64 & 79.60 & 87.13 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.01}&
*&*&*&*&
38.46 & 32.66 & 74.80 & 76.20 &
39.09 & 41.97 & 81.27 & 84.93 &
*&*&*&*\\
\midrule
\textsc{w/-rost-ep30-bs64}&&&&&&&&&&&&&\\
\textsc{lrd1e-2-wd0.1}&
*&*&*&*&
32.58 & 43.59 & 65.93 & 83.73 &
36.37 & 41.13 & 72.47 & 83.93 &
*&*&*&*\\
\textsc{lrd1e-3-wd0.1}&
*&*&*&*&
*&*&*&*&
38.55 & 38.54 & 71.13 & 84.07 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.1}&
27.12 & 48.38 & 58.07 & 84.27 &
33.40 & 42.21 & 65.67 & 83.73 &
36.70 & 40.59 & 69.80 & 84.53 &
33.94 & 48.10 & 78.87 & 86.13\\
&&&&&&&&&&&&&\\
\textsc{lrd1e-4-wd1.0}&
*&*&*&*&
29.21 & 49.88 & 72.67 & 80.60 &
25.93 & 54.88 & 75.73 & 81.13 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.5}&
*&*&*&*&
31.97 & 48.38 & 72.53 & 80.80 &
ai10&*&*&*&*&*&*&*\\
\textsc{lrd1e-4-wd0.2}&
*&*&*&*&
28.16 & 51.12 & 64.40 & 83.67 &
34.00 & 45.62 & 73.67 & 84.13 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.05}&
*&*&*&*&
35.91 & 30.36 & 65.93 & 78.20 &
40.06 & 32.22 & 72.20 & 79.60 &
*&*&*&*\\
\textsc{lrd1e-4-wd0.01}&
*&*&*&*&
29.50 & 28.89 & 63.33 & 66.80 &
34.45 & 32.48 & 72.60 & 72.73 &
*&*&*&*\\
\textsc{w/-rost-ep50-bs64}&&&&&&&&&&&&&\\
\bottomrule
\end{tabular}
}
\vspace{-0.2in}
\end{table*}


==> materials/tables/5_ours_table.tex <==
\begin{figure*}
\begin{center}
\noindent\begin{minipage}{.65\textwidth}
\begin{small}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccc}
\toprule
\multicolumn{1}{c}{\textsc{Pre-training}}&\multicolumn{4}{c}{\textsc{Continual Pre-training \& Fine-tuning}}\\
\multicolumn{1}{c}{\textsc{T0$\rightarrow$T4}}&\multicolumn{4}{c}{T5$\rightarrow$T8}\\
\midrule
& \textsc{T5}& \textsc{T6}& \textsc{T7}& \textsc{T8}\\
\midrule

\textsc{Supervised Learning} & 
{64.56} / 86.02 & 
{69.06} / 89.98 &
{75.06} / 91.44 & 
{77.80} / 93.86 \\
\cdashlinelr{1-5}
\textsc{+ GLAD (Ours)} & 
\textbf{65.78} / \textbf{86.84} & 
\textbf{69.84} / \textbf{90.52} & 
\textbf{76.12} / \textbf{91.76} & 
\textbf{79.04} / \textbf{94.54} \\
\midrule
\midrule

\textsc{SimMIM}~{\cite{xie2021simmim}} & 
\textbf{68.34} / 88.24 & 
{72.22} / 91.78 & 
{77.38} / 93.22 & 
{80.12} / 94.74 \\
\cdashlinelr{1-5}
\textsc{+ GLAD (Ours)} & 
{68.24} / \textbf{88.46} & 
\textbf{73.24} / \textbf{92.10} & 
\textbf{78.94} / \textbf{93.46} & 
\textbf{81.62} / \textbf{95.22} \\
\midrule
\midrule

\textsc{MAE}~{\small \cite{he2022masked}} & 
\textbf{42.19} / \textbf{70.01} & 
{52.07} / 78.56 & 
{63.07} / 85.38 & 
{71.19} / 90.94 \\
\cdashlinelr{1-5}
\textsc{+ GLAD (Ours)} & 
% {41.89} / 69.05 & 
% \textbf{53.67} / \textbf{79.94} & 
% \textbf{66.01} / \textbf{86.86} & 
% \textbf{73.51} / \textbf{91.72} \\
{41.75} / 69.46 & 
\textbf{54.74} / \textbf{80.84} & 
\textbf{68.01} / \textbf{87.59} & 
\textbf{74.30} / \textbf{92.19} \\
\bottomrule
\end{tabular}}
\end{small}
\end{minipage}
\hspace{0.1in}
\begin{minipage}{.3\textwidth}
\includegraphics[height=4cm]{figures/partial_layer_freeze.pdf} 
\end{minipage}
\vspace{-0.1in}
\caption{\footnotesize \textbf{Left: Per-task fine-tuning (top-1 / top-5) performance on T5 to T8 during continual pre-training} with base frameworks and our proposed method. \textbf{Right: Analysis for freezing the weights on a few lower/deeper layers during continual pre-training} after pre-training first task. We use supervised (\emph{Sup}) and masked image modeling (\emph{MIM}). \emph{LF} and \emph{DF} denote \emph{freezing lower layers} and \emph{freezing deeper layers}, respectively.}
\label{fig:glad-results}
\end{center}
\vspace{-0.1in}
\end{figure*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

